Keep That Card in Mind: Card Guessing with Limited Memory

A card guessing game is played between two players, Guesser and Dealer. At the beginning of the game, the Dealer holds a deck of $n$ cards (labeled $1, ..., n$). For $n$ turns, the Dealer draws a card from the deck, the Guesser guesses which card was drawn, and then the card is discarded from the deck. The Guesser receives a point for each correctly guessed card. With perfect memory, a Guesser can keep track of all cards that were played so far and pick at random a card that has not appeared so far, yielding in expectation $\ln n$ correct guesses. With no memory, the best a Guesser can do will result in a single guess in expectation. We consider the case of a memory bounded Guesser that has $m < n$ memory bits. We show that the performance of such a memory bounded Guesser depends much on the behavior of the Dealer. In more detail, we show that there is a gap between the static case, where the Dealer draws cards from a properly shuffled deck or a prearranged one, and the adaptive case, where the Dealer draws cards thoughtfully, in an adversarial manner. Specifically: 1. We show a Guesser with $O(\log^2 n)$ memory bits that scores a near optimal result against any static Dealer. 2. We show that no Guesser with $m$ bits of memory can score better than $O(\sqrt{m})$ correct guesses, thus, no Guesser can score better than $\min \{\sqrt{m}, \ln n\}$, i.e., the above Guesser is optimal. 3. We show an efficient adaptive Dealer against which no Guesser with $m$ memory bits can make more than $\ln m + 2 \ln \log n + O(1)$ correct guesses in expectation. These results are (almost) tight, and we prove them using compression arguments that harness the guessing strategy for encoding.

==> parts/discussion/relation_to_mirror_games.tex <==
In this section we discuss the relation between Card Guessing and Mirror Game.

Recall the Mirror Game presented by Garg and Schneider~\cite{GS17}, where Alice (the first player) and Bob take turns saying a name of a card from a deck of size $2n$, and a player loses if this card was mentioned already by either one of the players.
When no more cards are left to say, then the result of the game is a draw.
Bob, who plays second, has a {\em low memory, simple, and efficient strategy called mirroring}.
Bob fixes any matching on the cards, and for every card said by Alice, Bob responds with the matched card.
This allows Bob to say in every turn a card that has not appeared yet, and in our terms, to yield a reasonable guess, and is assured not to lose.

The question at hand is how much memory Alice needs in order not to lose (i.e.\ assure a draw).
Garg and Schneider~\cite{GS17} showed that every deterministic ``winning" (drawing) strategy for Alice requires space that is linear in $n$.
They also showed a randomized strategy that draws with high probability ($1-{1 \over n}$) and requires $O(\sqrt n)$ bits of memory while relying on access to a secret random matching oracle.
Using a similar setting (with respect to the secret matching), Feige~\cite{Feige19} showed a randomized strategy for Alice that requires only $O(\log^3 n)$ bits of memory.
In fact, as we will show soon, Alice can supply her own matching while being {\em computationally efficient} and using $O(n \log n)$ bits of long lived randomness to produce reasonable guesses (or alternatively using cryptography and a small amount of long lived randomness while assuming computational limitation (poly time) on Bob).

This stands in contrast to our impossibility result on the adaptive Dealer that bounds the number of reasonable guesses by the Guesser's memory, regardless of run time, how much randomness she holds, and what cryptography she uses.
We present here a simplified computationally efficient version of Feige's construction that requires no access to a secret random matching but requires long lived randomness with random access for efficiency.

Our first point is that it is possible to construct a secret matching from more standard assumptions (long lived random bits or cryptographic ones).
Ristenpart and Yilek~\cite{RistenpartYilek2013} and Morris and Rogaway~\cite{MR2014} showed a transformation from (pseudo)random functions to (pseudo)random permutations that is secure {\em even if all the permutation is given to the distinguisher}.
Applying their constructions in our setting means using $O(n \log n)$ random bits (with random access) to construct a random permutation $\pi$ so that given $x$ it is possible to evaluate $\pi(x)$ on the fly (same for $\pi^{-1}(x)$), simply by looking at the randomness in $O(\log n)$ places and using $O(\log n)$ memory bits for intermediate calculations.
Naor and Reingold~\cite{NaorReingold2002} showed a construction that takes a permutation and its inverse and produces a permutation with any desired cycle structure\footnote{Naor and Reingold took a permutation $\pi$, and a permutation with the structure of choice $\sigma$ and returned $\pi^{-1} \circ \sigma \circ \pi$.}.
In particular, we can turn $\pi$ to an involution, i.e., a matching\footnote{For example, by taking $\sigma$ to be the involution $\sigma(1) = 2, \sigma(3) =4, \dots$}.
The construction also gives each pair an ``index" in $[n]$ that is retrievable from either member of the pair.
Therefore combining these two we get that Alice can have a secret matching provided she has either (i)  $O(n \log n)$ secret random bits with random access or (ii) A key to a pseudorandom function and Bob is computationally limited and cannot distinguish the results from random.


Having a secret matching with the above properties we discuss how to use the machinery of \Cref{sec_static_dealer:sec_random_subsets_guesser:sec_amplification} in order to suggest a strategy for Alice.
Alice will use her secret matching to imitate the mirror strategy of Bob, with an arbitrary starting point.
However, from time to time she will fail in that Bob will select as a response the matched card of the starting point, leaving her with no obvious response.
What she should do at this point is select a card that has not appeared yet as a new starting point.
For this she needs the equivalent of a reasonable guess.
How many time do we expect this to happen?
This is similar to card guessing with perfect memory, i.e.\ $\ln n$ times.
So Alice needs altogether $\ln n$ different reasonable guesses.

So in more detail, Alice uses her memory to allocate the $2n$ cards to subsets, similarly to what we did in \Cref{sec_static_dealer:sec_random_subsets_guesser:sec_amplification}.
She uses her long lived randomness to sample~$O(\log^2 n)$ functions from a family of pairwise independent functions and splits the functions to $\log n$ collections of equal size. The $j$th collection
%The functions from the $j$th collection will be used to assign cards to subsets of size $2^{j-1}$.
%Each function is assigned to a different set size $2^j$, such that each $j$ has equal number of functions assigned to
A byproduct of Naor and Reingold's construction\cite{NaorReingold2002} is having an order on the pairs in the matching\footnote{In the above example, the first pair is $(1,2)$, the second is $(3,4)$, and so fourth.}.
Alice uses that order to assign matched cards to subsets.
For every function $\kwisefunc$ in the $j$th collection, Alice assigns the cards of the $i$th pair to the subset~$\jthsubseth$ if $\kwisefunc(i) \in \{2^{j-1}+1, \dots, 2^j\}$.
For each subset, Alice tracks the number of cards that appeared from that subset and ``remember the last card'', exactly as we did for our Randomized-Subset.

As her first card, Alice chooses an arbitrary card $g_1$, announce $g_1$ as her choice and stores it in her memory.
When Bob says a card $x$, Alice responds with $M(x)$, where $M$ is her secret matching.
She does that until Bob says $M(g_1)$.
Alice cannot say $M(M(g_1)) = g_1$, as this would result in her loosing.
So instead, she attempts to recover a {\em reasonable guess} from her memory.
If the recovering attempt succeeds and she retrieves card $g_2$, then she announces $g_2$ as her choice and stores it in her memory in place of $g_1$.
She continues until Bob says $M(g_2)$  and so forth.


So we get that Alice loses the game only in case she fails to recover a reasonable card when Bob makes a good guess.
Regarding the first half of the game, we can store a few singletons, cards that have not appeared (i.e.\ subsets of size $1$).
In the second half of the game, failure happens either if Alice has bad luck and her subsets don't yield sufficiently many reasonable guesses, or if Bob guesses correctly too many times and Alice doesn't have enough subsets.

When $\turnix \le n/2$th turns are left for Alice, she makes a recovery attempt from the collection of $j$th subsets such that $j = \log (n /2 \turnix)$.
She checks the subsets in some order until she finds one that yields a reasonable guess.
For the analysis, assume that Alice accesses each subset exactly once.
Afterward, that subset is deleted and ignored for the rest of the game, regardless of whether a recovery occurred.
From \Cref{claim_amplified_random_subset_yields_a_reasonable_guess}, we know that each subset yields a reasonable guess with constant probability.
As a result, Alice is expected to ``burn'' $O(1)$ subsets until she finds a good one. , and thus, she is expected to produce $O(\log n)$ reasonable guesses.
By a Chernoff bound, the probability she fails to produce $O(\log n)$ reasonable guesses is less than $1/ poly(n)$.

A different failure happens in case too many recovery attempts occur while Alice considers a specific $j$.
That is, when Alice ``burned" all $O(\log n)$ corresponding subsets.
In other words, in case Bob guesses correctly more than $O(\log n)$ times, while Alice considers the $j$th collection.
As Alice's matching is (pseudo)random, and since all of Bob's guesses are reasonable, we expect Bob to make no more than $O(1)$ correct guesses while Alice considers a specific $j$.
By a Chernoff, Bob makes $O(\log n)$ correct guess at that period in probability at most $1/poly(n)$.

As Alice wins only if no failure occurred during any of the $\log n$ periods, it follows that Alice wins with probability at least $1 - {\log n \over poly(n)} \ge 1 - {1 \over n}$.
We conclude that with $O(\log^3 n)$ bits of memory, $O(\log^2 n + n \log n)$ bits of long lasting randomness,  Alice has a winning strategy against (a computationally bounded) Bob, that draws with probability $1 - {1 \over n}$.
If we wish to go use computational assumptions, then Alice needs only to store a key to a pseudo-random function and we get the desired result.

Two interesting questions are (i) whether any of this is possible with at most polylog long lived bits of randomness and without cryptographic assumptions (ii) is the $\Omega(\log^2 n)$ lower bound of Section \ref{sec_static_dealer:upper_bound} relevant for this setting as well.  
